Reprompting: Automated Chain-of-Thought Prompt Inference Through Gibbs Sampling

We introduce Reprompting, an iterative sampling algorithm that automatically learns the Chain-of-Thought (CoT) recipes for a given task without human intervention. Through Gibbs sampling, Reprompting infers the CoT recipes that work consistently well for a set of training samples by iteratively sampling new recipes using previously sampled recipes as parent prompts to solve other training problems. We conduct extensive experiments on 20 challenging reasoning tasks. Results show that Reprompting outperforms human-written CoT prompts substantially by +9.4 points on average. It also achieves consistently better performance than the state-of-the-art prompt optimization and decoding algorithms.

==> math_commands.tex <==
%%%%% NEW MATH DEFINITIONS %%%%%

\usepackage{amsmath,amsfonts,bm}

% Mark sections of captions for referring to divisions of figures
\newcommand{\figleft}{{\em (Left)}}
\newcommand{\figcenter}{{\em (Center)}}
\newcommand{\figright}{{\em (Right)}}
\newcommand{\figtop}{{\em (Top)}}
\newcommand{\figbottom}{{\em (Bottom)}}
\newcommand{\captiona}{{\em (a)}}
\newcommand{\captionb}{{\em (b)}}
\newcommand{\captionc}{{\em (c)}}
\newcommand{\captiond}{{\em (d)}}

% Highlight a newly defined term
\newcommand{\newterm}[1]{{\bf #1}}


% Figure reference, lower-case.
\def\figref#1{figure~\ref{#1}}
% Figure reference, capital. For start of sentence
\def\Figref#1{Figure~\ref{#1}}
\def\twofigref#1#2{figures \ref{#1} and \ref{#2}}
\def\quadfigref#1#2#3#4{figures \ref{#1}, \ref{#2}, \ref{#3} and \ref{#4}}
% Section reference, lower-case.
\def\secref#1{section~\ref{#1}}
% Section reference, capital.
\def\Secref#1{Section~\ref{#1}}
% Reference to two sections.
\def\twosecrefs#1#2{sections \ref{#1} and \ref{#2}}
% Reference to three sections.
\def\secrefs#1#2#3{sections \ref{#1}, \ref{#2} and \ref{#3}}
% Reference to an equation, lower-case.
\def\eqref#1{equation~\ref{#1}}
% Reference to an equation, upper case
\def\Eqref#1{Equation~\ref{#1}}
% A raw reference to an equation---avoid using if possible
\def\plaineqref#1{\ref{#1}}
% Reference to a chapter, lower-case.
\def\chapref#1{chapter~\ref{#1}}
% Reference to an equation, upper case.
\def\Chapref#1{Chapter~\ref{#1}}
% Reference to a range of chapters
\def\rangechapref#1#2{chapters\ref{#1}--\ref{#2}}
% Reference to an algorithm, lower-case.
\def\algref#1{algorithm~\ref{#1}}
% Reference to an algorithm, upper case.
\def\Algref#1{Algorithm~\ref{#1}}
\def\twoalgref#1#2{algorithms \ref{#1} and \ref{#2}}
\def\Twoalgref#1#2{Algorithms \ref{#1} and \ref{#2}}
% Reference to a part, lower case
\def\partref#1{part~\ref{#1}}
% Reference to a part, upper case
\def\Partref#1{Part~\ref{#1}}
\def\twopartref#1#2{parts \ref{#1} and \ref{#2}}

\def\ceil#1{\lceil #1 \rceil}
\def\floor#1{\lfloor #1 \rfloor}
\def\1{\bm{1}}
\newcommand{\train}{\mathcal{D}}
\newcommand{\valid}{\mathcal{D_{\mathrm{valid}}}}
\newcommand{\test}{\mathcal{D_{\mathrm{test}}}}

\def\eps{{\epsilon}}


% Random variables
\def\reta{{\textnormal{$\eta$}}}
\def\ra{{\textnormal{a}}}
\def\rb{{\textnormal{b}}}
\def\rc{{\textnormal{c}}}
\def\rd{{\textnormal{d}}}
\def\re{{\textnormal{e}}}
\def\rf{{\textnormal{f}}}
\def\rg{{\textnormal{g}}}
\def\rh{{\textnormal{h}}}
\def\ri{{\textnormal{i}}}
\def\rj{{\textnormal{j}}}
\def\rk{{\textnormal{k}}}
\def\rl{{\textnormal{l}}}
% rm is already a command, just don't name any random variables m
\def\rn{{\textnormal{n}}}
\def\ro{{\textnormal{o}}}
\def\rp{{\textnormal{p}}}
\def\rq{{\textnormal{q}}}
\def\rr{{\textnormal{r}}}
\def\rs{{\textnormal{s}}}
\def\rt{{\textnormal{t}}}
\def\ru{{\textnormal{u}}}
\def\rv{{\textnormal{v}}}
\def\rw{{\textnormal{w}}}
\def\rx{{\textnormal{x}}}
\def\ry{{\textnormal{y}}}
\def\rz{{\textnormal{z}}}

% Random vectors
\def\rvepsilon{{\mathbf{\epsilon}}}
\def\rvtheta{{\mathbf{\theta}}}
\def\rva{{\mathbf{a}}}
\def\rvb{{\mathbf{b}}}
\def\rvc{{\mathbf{c}}}
\def\rvd{{\mathbf{d}}}
\def\rve{{\mathbf{e}}}
\def\rvf{{\mathbf{f}}}
\def\rvg{{\mathbf{g}}}
\def\rvh{{\mathbf{h}}}
\def\rvu{{\mathbf{i}}}
\def\rvj{{\mathbf{j}}}
\def\rvk{{\mathbf{k}}}
\def\rvl{{\mathbf{l}}}
\def\rvm{{\mathbf{m}}}
\def\rvn{{\mathbf{n}}}
\def\rvo{{\mathbf{o}}}
\def\rvp{{\mathbf{p}}}
\def\rvq{{\mathbf{q}}}
\def\rvr{{\mathbf{r}}}
\def\rvs{{\mathbf{s}}}
\def\rvt{{\mathbf{t}}}
\def\rvu{{\mathbf{u}}}
\def\rvv{{\mathbf{v}}}
\def\rvw{{\mathbf{w}}}
\def\rvx{{\mathbf{x}}}
\def\rvy{{\mathbf{y}}}
\def\rvz{{\mathbf{z}}}

% Elements of random vectors
\def\erva{{\textnormal{a}}}
\def\ervb{{\textnormal{b}}}
\def\ervc{{\textnormal{c}}}
\def\ervd{{\textnormal{d}}}
\def\erve{{\textnormal{e}}}
\def\ervf{{\textnormal{f}}}
\def\ervg{{\textnormal{g}}}
\def\ervh{{\textnormal{h}}}
\def\ervi{{\textnormal{i}}}
\def\ervj{{\textnormal{j}}}
\def\ervk{{\textnormal{k}}}
\def\ervl{{\textnormal{l}}}
\def\ervm{{\textnormal{m}}}
\def\ervn{{\textnormal{n}}}
\def\ervo{{\textnormal{o}}}
\def\ervp{{\textnormal{p}}}
\def\ervq{{\textnormal{q}}}
\def\ervr{{\textnormal{r}}}
\def\ervs{{\textnormal{s}}}
\def\ervt{{\textnormal{t}}}
\def\ervu{{\textnormal{u}}}
\def\ervv{{\textnormal{v}}}
\def\ervw{{\textnormal{w}}}
\def\ervx{{\textnormal{x}}}
\def\ervy{{\textnormal{y}}}
\def\ervz{{\textnormal{z}}}

% Random matrices
\def\rmA{{\mathbf{A}}}
\def\rmB{{\mathbf{B}}}
\def\rmC{{\mathbf{C}}}
\def\rmD{{\mathbf{D}}}
\def\rmE{{\mathbf{E}}}
\def\rmF{{\mathbf{F}}}
\def\rmG{{\mathbf{G}}}
\def\rmH{{\mathbf{H}}}
\def\rmI{{\mathbf{I}}}
\def\rmJ{{\mathbf{J}}}
\def\rmK{{\mathbf{K}}}
\def\rmL{{\mathbf{L}}}
\def\rmM{{\mathbf{M}}}
\def\rmN{{\mathbf{N}}}
\def\rmO{{\mathbf{O}}}
\def\rmP{{\mathbf{P}}}
\def\rmQ{{\mathbf{Q}}}
\def\rmR{{\mathbf{R}}}
\def\rmS{{\mathbf{S}}}
\def\rmT{{\mathbf{T}}}
\def\rmU{{\mathbf{U}}}
\def\rmV{{\mathbf{V}}}
\def\rmW{{\mathbf{W}}}
\def\rmX{{\mathbf{X}}}
\def\rmY{{\mathbf{Y}}}
\def\rmZ{{\mathbf{Z}}}

% Elements of random matrices
\def\ermA{{\textnormal{A}}}
\def\ermB{{\textnormal{B}}}
\def\ermC{{\textnormal{C}}}
\def\ermD{{\textnormal{D}}}
\def\ermE{{\textnormal{E}}}
\def\ermF{{\textnormal{F}}}
\def\ermG{{\textnormal{G}}}
\def\ermH{{\textnormal{H}}}
\def\ermI{{\textnormal{I}}}
\def\ermJ{{\textnormal{J}}}
\def\ermK{{\textnormal{K}}}
\def\ermL{{\textnormal{L}}}
\def\ermM{{\textnormal{M}}}
\def\ermN{{\textnormal{N}}}
\def\ermO{{\textnormal{O}}}
\def\ermP{{\textnormal{P}}}
\def\ermQ{{\textnormal{Q}}}
\def\ermR{{\textnormal{R}}}
\def\ermS{{\textnormal{S}}}
\def\ermT{{\textnormal{T}}}
\def\ermU{{\textnormal{U}}}
\def\ermV{{\textnormal{V}}}
\def\ermW{{\textnormal{W}}}
\def\ermX{{\textnormal{X}}}
\def\ermY{{\textnormal{Y}}}
\def\ermZ{{\textnormal{Z}}}

% Vectors
\def\vzero{{\bm{0}}}
\def\vone{{\bm{1}}}
\def\vmu{{\bm{\mu}}}
\def\vtheta{{\bm{\theta}}}
\def\va{{\bm{a}}}
\def\vb{{\bm{b}}}
\def\vc{{\bm{c}}}
\def\vd{{\bm{d}}}
\def\ve{{\bm{e}}}
\def\vf{{\bm{f}}}
\def\vg{{\bm{g}}}
\def\vh{{\bm{h}}}
\def\vi{{\bm{i}}}
\def\vj{{\bm{j}}}
\def\vk{{\bm{k}}}
\def\vl{{\bm{l}}}
\def\vm{{\bm{m}}}
\def\vn{{\bm{n}}}
\def\vo{{\bm{o}}}
\def\vp{{\bm{p}}}
\def\vq{{\bm{q}}}
\def\vr{{\bm{r}}}
\def\vs{{\bm{s}}}
\def\vt{{\bm{t}}}
\def\vu{{\bm{u}}}
\def\vv{{\bm{v}}}
\def\vw{{\bm{w}}}
\def\vx{{\bm{x}}}
\def\vy{{\bm{y}}}
\def\vz{{\bm{z}}}

% Elements of vectors
\def\evalpha{{\alpha}}
\def\evbeta{{\beta}}
\def\evepsilon{{\epsilon}}
\def\evlambda{{\lambda}}
\def\evomega{{\omega}}
\def\evmu{{\mu}}
\def\evpsi{{\psi}}
\def\evsigma{{\sigma}}
\def\evtheta{{\theta}}
\def\eva{{a}}
\def\evb{{b}}
\def\evc{{c}}
\def\evd{{d}}
\def\eve{{e}}
\def\evf{{f}}
\def\evg{{g}}
\def\evh{{h}}
\def\evi{{i}}
\def\evj{{j}}
\def\evk{{k}}
\def\evl{{l}}
\def\evm{{m}}
\def\evn{{n}}
\def\evo{{o}}
\def\evp{{p}}
\def\evq{{q}}
\def\evr{{r}}
\def\evs{{s}}
\def\evt{{t}}
\def\evu{{u}}
\def\evv{{v}}
\def\evw{{w}}
\def\evx{{x}}
\def\evy{{y}}
\def\evz{{z}}

% Matrix
\def\mA{{\bm{A}}}
\def\mB{{\bm{B}}}
\def\mC{{\bm{C}}}
\def\mD{{\bm{D}}}
\def\mE{{\bm{E}}}
\def\mF{{\bm{F}}}
\def\mG{{\bm{G}}}
\def\mH{{\bm{H}}}
\def\mI{{\bm{I}}}
\def\mJ{{\bm{J}}}
\def\mK{{\bm{K}}}
\def\mL{{\bm{L}}}
\def\mM{{\bm{M}}}
\def\mN{{\bm{N}}}
\def\mO{{\bm{O}}}
\def\mP{{\bm{P}}}
\def\mQ{{\bm{Q}}}
\def\mR{{\bm{R}}}
\def\mS{{\bm{S}}}
\def\mT{{\bm{T}}}
\def\mU{{\bm{U}}}
\def\mV{{\bm{V}}}
\def\mW{{\bm{W}}}
\def\mX{{\bm{X}}}
\def\mY{{\bm{Y}}}
\def\mZ{{\bm{Z}}}
\def\mBeta{{\bm{\beta}}}
\def\mPhi{{\bm{\Phi}}}
\def\mLambda{{\bm{\Lambda}}}
\def\mSigma{{\bm{\Sigma}}}

% Tensor
\DeclareMathAlphabet{\mathsfit}{\encodingdefault}{\sfdefault}{m}{sl}
\SetMathAlphabet{\mathsfit}{bold}{\encodingdefault}{\sfdefault}{bx}{n}
\newcommand{\tens}[1]{\bm{\mathsfit{#1}}}
\def\tA{{\tens{A}}}
\def\tB{{\tens{B}}}
\def\tC{{\tens{C}}}
\def\tD{{\tens{D}}}
\def\tE{{\tens{E}}}
\def\tF{{\tens{F}}}
\def\tG{{\tens{G}}}
\def\tH{{\tens{H}}}
\def\tI{{\tens{I}}}
\def\tJ{{\tens{J}}}
\def\tK{{\tens{K}}}
\def\tL{{\tens{L}}}
\def\tM{{\tens{M}}}
\def\tN{{\tens{N}}}
\def\tO{{\tens{O}}}
\def\tP{{\tens{P}}}
\def\tQ{{\tens{Q}}}
\def\tR{{\tens{R}}}
\def\tS{{\tens{S}}}
\def\tT{{\tens{T}}}
\def\tU{{\tens{U}}}
\def\tV{{\tens{V}}}
\def\tW{{\tens{W}}}
\def\tX{{\tens{X}}}
\def\tY{{\tens{Y}}}
\def\tZ{{\tens{Z}}}


% Graph
\def\gA{{\mathcal{A}}}
\def\gB{{\mathcal{B}}}
\def\gC{{\mathcal{C}}}
\def\gD{{\mathcal{D}}}
\def\gE{{\mathcal{E}}}
\def\gF{{\mathcal{F}}}
\def\gG{{\mathcal{G}}}
\def\gH{{\mathcal{H}}}
\def\gI{{\mathcal{I}}}
\def\gJ{{\mathcal{J}}}
\def\gK{{\mathcal{K}}}
\def\gL{{\mathcal{L}}}
\def\gM{{\mathcal{M}}}
\def\gN{{\mathcal{N}}}
\def\gO{{\mathcal{O}}}
\def\gP{{\mathcal{P}}}
\def\gQ{{\mathcal{Q}}}
\def\gR{{\mathcal{R}}}
\def\gS{{\mathcal{S}}}
\def\gT{{\mathcal{T}}}
\def\gU{{\mathcal{U}}}
\def\gV{{\mathcal{V}}}
\def\gW{{\mathcal{W}}}
\def\gX{{\mathcal{X}}}
\def\gY{{\mathcal{Y}}}
\def\gZ{{\mathcal{Z}}}

% Sets
\def\sA{{\mathbb{A}}}
\def\sB{{\mathbb{B}}}
\def\sC{{\mathbb{C}}}
\def\sD{{\mathbb{D}}}
% Don't use a set called E, because this would be the same as our symbol
% for expectation.
\def\sF{{\mathbb{F}}}
\def\sG{{\mathbb{G}}}
\def\sH{{\mathbb{H}}}
\def\sI{{\mathbb{I}}}
\def\sJ{{\mathbb{J}}}
\def\sK{{\mathbb{K}}}
\def\sL{{\mathbb{L}}}
\def\sM{{\mathbb{M}}}
\def\sN{{\mathbb{N}}}
\def\sO{{\mathbb{O}}}
\def\sP{{\mathbb{P}}}
\def\sQ{{\mathbb{Q}}}
\def\sR{{\mathbb{R}}}
\def\sS{{\mathbb{S}}}
\def\sT{{\mathbb{T}}}
\def\sU{{\mathbb{U}}}
\def\sV{{\mathbb{V}}}
\def\sW{{\mathbb{W}}}
\def\sX{{\mathbb{X}}}
\def\sY{{\mathbb{Y}}}
\def\sZ{{\mathbb{Z}}}

% Entries of a matrix
\def\emLambda{{\Lambda}}
\def\emA{{A}}
\def\emB{{B}}
\def\emC{{C}}
\def\emD{{D}}
\def\emE{{E}}
\def\emF{{F}}
\def\emG{{G}}
\def\emH{{H}}
\def\emI{{I}}
\def\emJ{{J}}
\def\emK{{K}}
\def\emL{{L}}
\def\emM{{M}}
\def\emN{{N}}
\def\emO{{O}}
\def\emP{{P}}
\def\emQ{{Q}}
\def\emR{{R}}
\def\emS{{S}}
\def\emT{{T}}
\def\emU{{U}}
\def\emV{{V}}
\def\emW{{W}}
\def\emX{{X}}
\def\emY{{Y}}
\def\emZ{{Z}}
\def\emSigma{{\Sigma}}

% entries of a tensor
% Same font as tensor, without \bm wrapper
\newcommand{\etens}[1]{\mathsfit{#1}}
\def\etLambda{{\etens{\Lambda}}}
\def\etA{{\etens{A}}}
\def\etB{{\etens{B}}}
\def\etC{{\etens{C}}}
\def\etD{{\etens{D}}}
\def\etE{{\etens{E}}}
\def\etF{{\etens{F}}}
\def\etG{{\etens{G}}}
\def\etH{{\etens{H}}}
\def\etI{{\etens{I}}}
\def\etJ{{\etens{J}}}
\def\etK{{\etens{K}}}
\def\etL{{\etens{L}}}
\def\etM{{\etens{M}}}
\def\etN{{\etens{N}}}
\def\etO{{\etens{O}}}
\def\etP{{\etens{P}}}
\def\etQ{{\etens{Q}}}
\def\etR{{\etens{R}}}
\def\etS{{\etens{S}}}
\def\etT{{\etens{T}}}
\def\etU{{\etens{U}}}
\def\etV{{\etens{V}}}
\def\etW{{\etens{W}}}
\def\etX{{\etens{X}}}
\def\etY{{\etens{Y}}}
\def\etZ{{\etens{Z}}}

% The true underlying data generating distribution
\newcommand{\pdata}{p_{\rm{data}}}
% The empirical distribution defined by the training set
\newcommand{\ptrain}{\hat{p}_{\rm{data}}}
\newcommand{\Ptrain}{\hat{P}_{\rm{data}}}
% The model distribution
\newcommand{\pmodel}{p_{\rm{model}}}
\newcommand{\Pmodel}{P_{\rm{model}}}
\newcommand{\ptildemodel}{\tilde{p}_{\rm{model}}}
% Stochastic autoencoder distributions
\newcommand{\pencode}{p_{\rm{encoder}}}
\newcommand{\pdecode}{p_{\rm{decoder}}}
\newcommand{\precons}{p_{\rm{reconstruct}}}

\newcommand{\laplace}{\mathrm{Laplace}} % Laplace distribution

\newcommand{\E}{\mathbb{E}}
\newcommand{\Ls}{\mathcal{L}}
\newcommand{\R}{\mathbb{R}}
\newcommand{\emp}{\tilde{p}}
\newcommand{\lr}{\alpha}
\newcommand{\reg}{\lambda}
\newcommand{\rect}{\mathrm{rectifier}}
\newcommand{\softmax}{\mathrm{softmax}}
\newcommand{\sigmoid}{\sigma}
\newcommand{\softplus}{\zeta}
\newcommand{\KL}{D_{\mathrm{KL}}}
\newcommand{\Var}{\mathrm{Var}}
\newcommand{\standarderror}{\mathrm{SE}}
\newcommand{\Cov}{\mathrm{Cov}}
% Wolfram Mathworld says $L^2$ is for function spaces and $\ell^2$ is for vectors
% But then they seem to use $L^2$ for vectors throughout the site, and so does
% wikipedia.
\newcommand{\normlzero}{L^0}
\newcommand{\normlone}{L^1}
\newcommand{\normltwo}{L^2}
\newcommand{\normlp}{L^p}
\newcommand{\normmax}{L^\infty}

\newcommand{\parents}{Pa} % See usage in notation.tex. Chosen to match Daphne's book.

\DeclareMathOperator*{\argmax}{arg\,max}
\DeclareMathOperator*{\argmin}{arg\,min}

\DeclareMathOperator{\sign}{sign}
\DeclareMathOperator{\Tr}{Tr}
\let\ab\allowbreak


==> old_approach.tex <==
\section{\codename: Prompt Inference Through Gibbs Sampling}
\subsection{Statistical Assumptions Behind In-Context Learning}
 \textbf{In-context learning} has become the cornerstone of evaluating large language models (LLMs) \citep{gpt3,srivastava2022beyond}. To facilitate this evaluation approach, data is provided for a large number of different tasks, with each task consisting of dozens or, more often, hundreds of instances with varying problem setup and question texts $x_i$ and their corresponding text answers $y_i$, where $i\in [1..N]$ and $N$ is the number of problem instances for the task. Statistically, in-context learning is based on the following assumption (which was verified empirically in \cite{gpt3}): 
\begin{equation}
    p_{LLM}(y_j | \{x_i, y_i\}_{i \neq j}, x_j) \approx p_{LLM}(y_j | \{x_i, y_i\}_{i \in S_j}, x_j), \quad \forall S_j \subset [1,N] \backslash \{j\}, |S_j|=K
\end{equation}
that is, the probability~$p_{LLM}(y_j | \{x_i, y_i\}_{i \in S_j}, x_j)$ of a given LLM generating the answer text~$y_j$ when prompted with the concatenation of the few-shot examples~$\{x_i, y_i\}_{i \in S_j \subset [1,N] \backslash \{j\}}$ and the test question~$x_j$ (i.e. $[x_{S_j^1}, y_{S_j^1}, ..., x_{S_j^K}, y_{S_j^K}, x_j]$) is close to the probability~$p_{LLM}(y_j | \{x_i, y_i\}_{i \neq j}, x_j)$ conditioned on all training examples~$\{x_i, y_i\}_{i \neq j}$.
In other words, any collection of $K$ examples of question-answer pairs~$\{x_i, y_i\}_{i \in S_j}$ can be used as a prompt prior to the test question $x_j$ for an LLM to predict the answer~$y_j$. In practice, however, the choice and even the order of examples can have a substantial impact on the test performance~\citep{lu2022fantastically}. And more importantly, the performance can be significantly enhanced by incorporating auxiliary knowledge or human-written instructions in a prompt~\citep{shwartz-etal-2020-unsupervised,zelikman2022star,nye2021show}, particularly in the form of Chain-of-Thought (CoT) reasoning~\citep{wei2022chain, wang2022self, zhou2022least, creswell2022selection, wang2022rationale,liu-etal-2022-multi, kojima2022large, li2022advance}.

\begin{figure}[t]
    \centering
    \includegraphics[width=.48\textwidth]{figures/logical_deduction_chatgpt_zeroshot.png}
\caption{An example that ChatGPT can propose various different solutions to the same problem in zero-shot.}
\label{fig:zeroshot_solutions}
\end{figure}

In-context learning with CoT~\citep{wei2022chain} can be seen in a similar light, statistically. In addition to the question-answer pairs~$\{x_i, y_i\}$, the CoT prompt also contains worked out step-by-step reasoning ``recipes''~$z_i$ in text, which are inserted between the question and answer:~$\{x_i, z_i, y_i\}$. These recipes can play two roles. First, they further explain the intent of the question~$x_i$, as a small collection of question-answer pairs alone may be insufficient to disambiguate among different patterns an LLM might detect. The second role is more important: it provides step-by-step guidance on one problem and thus teaches an LLM to solve similar problems following the same routine as it continues the text conditioned on the previous tokens.
In the extreme, with prompts that strictly regiment self-attention, GPT models can be turned into Turing Machines to execute standard computer algorithms \citep{jojic2023gptTM}. In practice, the CoT prompts commonly used in prior work fall somewhere between colloquial explanations and regimented recipes. Formally, {\bf in-context learning with CoT} is based on the following assumption (which was empirically verified in~\cite{wei2022chain}):
\begin{equation}
    p_{LLM}(z_j, y_j | \{x_i, z_i, y_i\}_{i \neq j}, x_j, m) \approx p_{LLM}(z_j, y_j | \{x_i, z_i, y_i\}_{i \in S_j}, x_j, m), \quad \forall S_j \subset [1,N] \backslash \{j\}, |S_j|=K
\label{eq:in_context_assumption}
\end{equation}
that is, the probability $p_{LLM}(z_j, y_j | \{x_i, z_i, y_i\}_{i \in S_j}, x_j, m)$ of a given LLM generating a step-by-step solution~$z_j$ followed by the correct answer~$y_j$ when prompted with the concatenation of the few-shot examples with CoT~$\{x_i, z_i, y_i\}_{i \in S_j \subset [1,N] \backslash \{j\}}$, the test question~$x_j$, and a special message~$m$ (i.e. $[x_{S_j^1}, m, z_{S_j^1}, y_{S_j^1}, ..., x_{S_j^K}, m, z_{S_j^K}, y_{S_j^K}, x_j, m]$) is close to the probability~$p_{LLM}(z_j, y_j | \{x_i, z_i, y_i\}_{i \neq j}, x_j, m)$ conditioned on all training solutions~$\{x_i, z_i, y_i\}_{i \neq j}$. Here, the special message~$m$ is an instruction text that is independent of specific questions and is appended to each question text. It can be task-specific or generic, as in the case of our experiments. Specifically, we use the following message for all tasks:

$m=$ \small \verb=Let's think step by step. At the end, show your answer bracketed with=
\verb=  <answer> and </answer>. Finally generate END at the end of the solution.=\normalsize

This message instructs the model to generate the step-by-step solution~$z_j$ prior to the answer text~$y_j$ and the specific format to present the answer.\footnote{This enables us to separate the generated answer~$y_j$ from the step-by-step solution~$z_j$ and forces the model to stop after generating the answer.} In fact, such an instruction message can trigger instruction-tuned LLMs to generate step-by-step solutions given~$[x_j, m]$ alone without any demonstration examples~(i.e.~$K = 0$), as illustrated in Figure~\ref{fig:zeroshot_solutions}. These solutions follow varying styles and often lead to incorrect answers. However, we argue that good recipes for solving the set of problems on a given task can evolve from these zero-shot solutions. In the next section, we introduce \codename, an iterative sampling algorithm that automatically produces the CoT recipes for a given set of problems without human intervention.

\subsection{Prompt Inference Through Gibbs Sampling}
We introduce the \codename algorithm, which aims to find a set of CoT recipes~$z_i$ that work {\bf consistently} well as few-shot in-context examples for a dataset $\{x_i,y_i\}_{i=1}^N$. Specifically, we formulate it as the problem of sampling from a joint distribution
\begin{equation}
    p(z_1, z_2,...z_N| \{x_i,y_i\}_{i=1}^N, m)
\label{eq:joint_distribution}
\end{equation}
such that the conditional distributions~$p(z_j | z_1,...,z_{j-1},z_{j+1},...z_N, \{x_i,y_i\}_{i=1}^N, m)$ satisfy the in-context learning assumption~\eqref{eq:in_context_assumption} that enables generalization with few-shot examples, i.e. the probability $p_{LLM}(z_j, y_j | \{x_i, z_i, y_i\}_{i \in S_j}, x_j, m)$ under the LLM is high and approximately invariant to the choice of examples~$S_j$. 
Thus, we have the approximation
\begin{equation}
\begin{split}
    &p(z_j | z_1,...,z_{j-1},z_{j+1},...z_N, \{x_i,y_i\}_{i=1}^N, m) \\
    \propto& p_{LLM}(z_j, y_j | \{x_i, z_i, y_i\}_{i \neq j}, x_j, m) \\
    \approx& p_{LLM}(z_j, y_j | \{x_i, z_i, y_i\}_{i \in S_j}, x_j, m), \, \quad \forall S_j \subset [1,N]\backslash \{j\}, |S_j| = K
\end{split}
\label{eq:reprompting_approximation}
\end{equation}

Without characterizing the joint distribution, we can use Gibbs sampling~\citep{Geman1984StochasticRG} to generate such samples~$\{z_1, z_2,...z_N\}$ by first sampling~$\{z_1, z_2,...z_N\}$ independently from the distributions~$p(z_j | x_j, y_j)$, and then iteratively drawing samples from the conditional distributions~$p(z_j | z_1,...,z_{j-1},z_{j+1},...z_N, \{x_i,y_i\}_{i=1}^N, m)$. Based on the approximation~\eqref{eq:reprompting_approximation}, we can sample~$z_j$ by randomly picking $K$ data points~(excluding~$j$) and then sampling~$z_j$ with weights proportional to the conditional probability
\begin{equation}
\begin{split}
    p_{LLM}(z_j, y_j | \{x_i, z_i, y_i\}_{i \in S_j}, x_j, m) =& p_{LLM}(z_j | \{x_i, z_i, y_i\}_{i \in S_j}, x_j, m) \cdot p_{LLM}(y_j | \{x_i, z_i, y_i\}_{i \in S_j}, x_j, m, z_j)
\end{split}
\end{equation}
One way to approximate it is to sample several~$\hat{z}_j$ from the LLM conditioned on the concatenation~$[x_{S_j^1}, m, z_{S_j^1}, y_{S_j^1}, ..., x_{S_j^K}, m, z_{S_j^K}, y_{S_j^K}, x_j, m]$, compute the weight for each~$\hat{z}_j$ using the model's probability of the correct answer~$y_j$ conditioned on ~$[x_{S_j^1}, m, z_{S_j^1}, y_{S_j^1}, ..., x_{S_j^K}, m, z_{S_j^K}, y_{S_j^K}, x_j, m, \hat{z}_j]$, and sample a~$z_j$ from~$\{\hat{z}_j\}$ based on the weights. In practice, however, the model's probability of a given text may not be accessible. Thus, we approximately sample~$z_j$ by sampling~$\hat{z}_j$ and~$\hat{y}_j$ from~$p_{LLM}(z, y | \{x_i, z_i, y_i\}_{i \in S_j}, x_j, m)$ and then reject~$\hat{z}_j$ with a probability of~$p_{rej}$ if~$\hat{y}_j \neq y_j$. Otherwise, we accept~$\hat{z}_j$ and update the sample. 
Algorithm~\ref{alg:reprompting} shows the complete \codename algorithm consisting of the initialization and iterative sampling steps, which can be realized using different LLMs. Note that we set the rejection probability~$p_{rej}$ in a way that allows solutions that lead to incorrect answers to be kept occasionally, as these solutions may still contain useful segments that evolve into good recipes through \codename.

\begin{algorithm}[ht]
\DontPrintSemicolon
\SetKwInOut{Input}{Input}
\Input{Training set $\{x_i,y_i\}_{i=1}^N$, number of shots $K$, number of iterations $M$, rejection probability~$p_{rej}$, the initialization model~$LLM_1$ and the sampling model~$LLM_2$}
\textbf{Initialization:}\;
\For {each $j$}{
$z_j \leftarrow \emptyset$\;
Sample $\hat{z}_j, \hat{y}_j \sim p_{LLM_1}(z, y | x_j, m)$\;
Sample $u \sim Uniform([0, 1])$\;
\If {$\hat{y}_j = y_j$ or $u>p_{rej}$}{
$z_j \leftarrow \hat{z}_j$\;
}
}
\textbf{Sampling:}\;
\Repeat{convergence or $M$ iterations are reached}{
Randomly select $j \in [1, N]$\;
Randomly select $S_j \subset [1,N]\backslash \{j\}$ of size $K$\;
Sample $\hat{z}_j, \hat{y}_j \sim p_{LLM_2}(z, y | \{x_i, z_i, y_i\}_{i \in S_j}, x_j, m)$\;
Sample $u \sim Uniform([0, 1])$\;
\If {$\hat{y}_j = y_j$ or $u>p_{rej}$}{
$z_j \leftarrow \hat{z}_j$\;
}
}
\caption{\codename algorithm}
\label{alg:reprompting}
\end{algorithm}

Ideally, the algorithm should converge to the point where the probability $p_{LLM}(z_j, y_j | \{x_i, z_i, y_i\}_{i \in S_j}, x_j, m)$ is high and agnostic to the choice of~$S_j$, which leads to a set of~$\{z_j\}$ that work well as a prompt for solving similar problems in a separate test set.

The algorithm can also be viewed as a variant of evolutionary algorithms:~1) First, we generate the initial population of individuals (where each individual is a CoT recipe given a problem). 2) Next, we repeat the following regeneration steps iteratively: 2a) we first evaluate the fitness of each CoT recipe by comparing the answer that follows the recipe with the correct answer and weed out the least-fit recipes; 2b) we then breed new individuals through crossover and mutation by randomly selecting K recipes from the population as parent recipes, which are then used to prompt the LLM to generate recipes for a new problem. By repeating the 2a and 2b steps, initial recipes can be recombined~(Figure~\ref{fig:reprompt_combine_examples}) and evolve into better recipes (Figure~\ref{fig:reprompt_examples}) through iterations. And eventually, the fittest recipes (i.e. ones that lead to more accurate solutions) will survive.

During testing, we select~$K$ tuples~$\{x_i, z_i, y_i\}$ from the inferred~$\{z_j\}$ based on the training accuracy when using each tuple individually in a prompt.

% In addition, we introduce a variant of the algorithm with greedy search for faster convergence. In this variant, instead of selecting~$S_j$ randomly, we select~$K$ tuples~$\{x_i, z_i, y_i\}$ based on the training accuracy when using each tuple individually in a prompt. Also, we replace~$z_j$ with~$\hat{z}_j$ only if the tuple~$(x_j, \hat{z}_j, y_i)$ obtains higher training accuracy than~$(x_j, z_j, y_i)$ when used in a prompt.
